Quantum Optimal Control Theory

The control of quantum dynamics via specially tailored laser pulses is a long-standing goal in physics and chemistry. Partly, this dream has come true, as sophisticated pulse shaping experiments allow to coherently control product ratios of chemical reactions. The theoretical design of the laser pulse to transfer an initial state to a given final state can be achieved with the help of quantum optimal control theory (QOCT). This tutorial provides an introduction to QOCT. It shows how the control equations defining such an optimal pulse follow from the variation of a properly defined functional. We explain the most successful schemes to solve these control equations and show how to incorporate additional constraints in the pulse design. The algorithms are then applied to simple quantum systems and the obtained pulses are analyzed. Besides the traditional final-time control methods, the tutorial also presents an algorithm and an example to handle time-dependent control targets.

==> algorithm.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Algorithm}
\label{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In this section we present iterative schemes for the optimization of laser fields under additional constraints on the fluence and/or on the spectral distribution.
%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Fluence constraint}
%%%%%%%%%%%%%%%%%%%%%%%
%
We first describe the algorithm which yields an optimized laser pulse producing an assigned value of $E_{0_j}$ (for each polarization direction $j=x,y$, cf. equation \eref{eq:fluence}). The set of coupled equations to be solved is given by equations (\ref{eq:field}),  (\ref{eq:SE}), (\ref{eq:SE2}) and (\ref{eq:SE3}).
The scheme below shows the order in which these equations are solved in the $k$-th iterative step.
%
\begin{equation}
\label{eq:scheme}
%
\begin{array}{l c c l c c c c }
%
  {\mbox{k-th step:}} \,\, & \Psi^{(k)}(0) & \overset{{\bepsilon}^{(k)}(t)}{\longrightarrow} &
%
 \Psi^{(k)}(T) &  &  &  &\\
%%
%%
          & & & \left[ \Psi^{(k)}(T) \right. & \overset{{\bepsilon}^{(k)}(t)}{\longrightarrow} &
% 
 \left. \Psi^{(k)}(0) \right] & & \\
%%
%%
                   & & & \chi^{(k)}(T) & \overset{\widetilde{{\bepsilon}}^{(k)}(t) 
% 
}{\longrightarrow} & \chi^{(k)}(0), & &
%%
%
\end{array}
\end{equation}
%
with the laser fields $\bepsilon^{(k)}(t),\tilde{\bepsilon}^{(k)}(t)$ given by
%
\begin{eqnarray}
%
\label{eq:feld1}
%
\widetilde{\epsilon}_j^{(k)}(t) &=& -  \frac{1}{\alpha_j^{(k)}}\Im\langle\chi^{(k)}(t)|\hat{\mu}_j|\Psi^{(k)}(t)\rangle,\\
%%
%%
\label{eq:feld2}
%
\epsilon_j^{(k+1)}(t) &=& \frac{\alpha_j^{(k)} }{\alpha_j^{(k+1)}} \widetilde{\epsilon}_j^{(k)}(t), \qquad \qquad j=x,y,
%
\end{eqnarray}
%
where the Lagrange multiplier $\alpha^{(k+1)}_j$ is defined by:
%
\begin{eqnarray}
%
\label{eq:alpha1}
\alpha_j^{(k+1)} = \sqrt{\frac{\int_0^T \!\! dt  \left[ \alpha_j^{(k)} \widetilde{\epsilon}_j^{(k)}(t) \right]^2 }{E_{0_j}}}.
\end{eqnarray}
%
The initial conditions in every iteration step are
%
\begin{eqnarray}
%
\label{eq:initial_psi}
  \Psi({\bf r},0)&=& \phi({\bf r}),\\
%
\label{eq:initial_chi}
  \chi({\bf r},T) &=& \widehat{O} \Psi({\bf r},T).
%
\end{eqnarray}
%
%

The scheme starts with the propagation of $\Psi^{(0)}({\bf r},t)$ forward in time using the laser field $\epsilon^{(0)}(t)$ which has to be guessed. The result of the propagation is the wave-function $\Psi^{(0)}({ \bf r },T)$ which is now used to calculate $\chi^{(0)}({\bf r},T)$ by applying the target operator (\ref{eq:initial_chi}). We continue with propagating  $\chi^{(0)}({ \bf r },t)$ backwards in time using the laser field $\widetilde{\epsilon}^{(0)}(t)$ (\ref{eq:feld1}). To solve equation \eref{eq:feld1} we have to know both wave functions $\Psi^{(0)}({ \bf r },t)$ and $\chi^{(0)}({ \bf r },t)$ at the same time $t$, which makes it necessary to either store the whole time-dependent wave function $\Psi^{(0)}({ \bf r },t)$ or propagate it backwards with the previous laser field $\epsilon^{(0)}(t)$. The version of the algorithm that avoids storage is indicated by the brackets in the scheme (\ref{eq:scheme}). Besides that, it is necessary to provide an initial value for $\alpha_j^{(0)}$ which we choose to be:
%
\begin{eqnarray}
\nonumber
\alpha_j^{(0)} = \sqrt{\frac{\int_0^T \!\! dt \,\,  \left[\epsilon_j^{(0)}(t)\right]^2}{E_{0_j}}}.
\end{eqnarray}
%
The result of the backward propagation $\chi^{(0)}({ \bf r },t)$ is the laser field $\widetilde{\epsilon}^{(0)}(t)$ which we now re-scale to the right value (\ref{eq:feld2}) yielding $\epsilon^{(1)}(t)$. This completes the first step. The second $(k=1)$ or, in general, the $k$th iteration repeats the described procedure starting again from the initial state $\Psi^{(k)}({ \bf r },t)=\phi({\bf r})$ and applying the rescaled field $\epsilon^{(k)}(t)$.
%

The scheme described above has some aspects in common with the techniques described in reference \cite{K89} and reference \cite{ZBR98,ZR98}:
The basic idea of incorporating fluence constraints in the optimization algorithm was given in reference \cite{K89}. However, the authors do not make use of the immediate feedback (cf. equation \eref{eq:feld1}), i.e. the backward propagation is accomplished by updating $\chi({ \bf r },t)$ and $\epsilon(t)$ in a self-consistent way, which was suggested in reference \cite{ZBR98,ZR98}. On the other hand, the technique presented by the authors of reference \cite{ZBR98,ZR98} does not allow to fix the fluence to a given value.
Roughly speaking, the technique presented above is a combination of both approaches. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Spectral constraint}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The algorithm with built in spectral restrictions is similar to the one presented above with two important differences: The factor $\alpha_j$ is a penalty factor. It has to be specified from the start and remains unchanged during the optimization. Second, the update of the field $\epsilon_j^{(k+1)}(t)$ in equation \eref{eq:feld2} has to be replaced by:
%
\begin{eqnarray}
%
\label{eq:feld2_filter}
%
\epsilon_j^{(k+1)}(t) &=&  \mathcal{F}^{-1} \left[ f_j(\omega) \times \mathcal{F}\left[\widetilde{\epsilon}_j^{(k)}(t)\right]\right]  \qquad j=x,y,
%
\end{eqnarray}
%
where the symbol $\mathcal{F}$ indicates a Fourier-transform.
%
The spectral constraint is formulated in terms of a filter function $f_j(\omega)$. Since $\epsilon_j(t)$ is real valued we have to make sure that $f_j(\omega) = f_j(-\omega)$. For example, the filter function could be chosen to be: 
%
\begin{eqnarray}
%
\label{eq:filter1}
%
f_j(\omega) =  \exp[-\gamma (\omega-\omega_0)^2] + \exp[-\gamma (\omega+\omega_0)^2],
%
\end{eqnarray}
%
so that only the frequency components around the center, $\pm \omega_0$, of the Gaussians are allowed in the pulse. If one uses instead:
\begin{eqnarray}
%
\label{eq:filter2}
%
\tilde{f}_j(\omega) = 1- \left(\exp[-\gamma (\omega-\omega_0)^2] + \exp[-\gamma (\omega+\omega_0)^2]\right),
%
\end{eqnarray}
%
one would allow every spectral component in the laser field except the components around $\pm \omega_0$.\\
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Spectral and fluence constraint}
%%%%%%%%%%%%%%%%%%%%%%%%%
Finally, we note that both schemes can be combined. This combination makes it possible to incorporate even more realistic experimental constraints in computational pulse optimizations. 
This is achieved by the scheme (\ref{eq:scheme}), the equation (\ref{eq:feld1}) and:
%
\begin{eqnarray}
%
\label{eq:feld2_filter_fixed}
%
\bar{\epsilon}_j^{(k)}(t) &=&   \mathcal{F}^{-1} \left[ f_j(\omega) \times \mathcal{F}  \left[\widetilde{\epsilon}_j^{(k)}(t)\right]\right] \qquad j=x,y,\\
%
\label{eq:feld2_filter_fixed2}
\epsilon_j^{(k+1)}(t) &=&  \frac{\alpha_j^{(k)}}{\alpha_j^{(k+1)}} \bar{\epsilon}_j^{(k)}(t),
%
\end{eqnarray}
%
where $\alpha_j^{(k+1)} $ is evaluated with the filtered field $\bar{\epsilon}_j^{(k)}(t)$
\begin{eqnarray}
%
\label{eq:alpha_filterfixed}
\alpha_j^{(k+1)} = \sqrt{\frac{\int_0^T \!\! dt  \left[ \alpha_j^{(k)} \bar{\epsilon}_j^{(k)}(t) \right]^2 }{E_{0_j}}},
\end{eqnarray}
%
to yield the right value for  $E_{0_j}$. The total spectral power is related to the fluence Parseval's theorem:
%
\begin{eqnarray} 
%
\nonumber
%
E_{0_j} = \int_{-\infty}^{+\infty} \!\! dt \,\, \theta(t) \theta(T-t) \left[\epsilon_j(t)\right]^2 = \frac{1}{2 \pi} \int_{-\infty}^{+\infty} \!\! d\omega \,\, \left| \epsilon_j(\omega)\right|^2 
%
\end{eqnarray}
%

In this combined form we first apply the filter function to the laser field (\ref{eq:feld2_filter_fixed}) then we rescale the field to yield the right value for $E_{0_j}$ (see equation \eref{eq:feld2_filter_fixed2}).
%

We conclude the section with a few remarks:
%
\begin{itemize}
\item
For each polarization direction one can specify a separate filter or fluence.
%
\item
The convergence proofs of references \cite{ZBR98,ZR98} do not go through in our case. This is due to the changing value for $\alpha_j^{(k)}$ and, in the case of spectral constraints, due to the modified field (\ref{eq:feld2_filter}). However, as will be shown in \sref{sec:results}, we still find a very good convergence of the presented algorithms in the numerical examples. Even for the ``brute-force'' spectral filter we find a satisfying convergence behavior (if not too many essential features of the pulse are suppressed by the function $f_j(\omega)$).
%
\item
Note, that if the target operator is a projection operator, like in equation \eref{eq:target_proj} a different choice for the functional $J_3$ (\ref{eq:J3}) is possible, namely one can choose the functional \cite{ZBR98}:
\begin{eqnarray}
\tilde{J}_3[{ \bepsilon },\Psi,\chi] = - 2 \Im \left\{ \left\langle \Psi(T)| \phi_f \right\rangle \int_0^T\!\! dt \,\, \left\langle \chi(t) \left| \left(i \partial_t
  % 
    -\hat{H}\right) \right| \Psi(t) \right\rangle \right\}
\end{eqnarray}
If we choose this functional, the control equation \eref{eq:SE3} has to be replaced by:
\begin{eqnarray}
\label{eq:newSE3}
\chi({ \bf r },T) = \Phi_f({\bf r})
\end{eqnarray}
With this choice we have two options, namely we can start the algorithm by propagating the initial state $\Psi({\bf r},0)=\Phi_i({\bf r})$ forward in time, or we start with propagating $\chi({\bf r},T)=\Phi_f({\bf r})$ backwards, like it is done in reference \cite{ZBR98}.
We have chosen the functional $J_3$ (\ref{eq:J3}) because it is more general, i.e., also the local target operator can be used. 
\item 
Since we do not expect a monotonic convergence we have to add some additional intelligence to the algorithm, e.g. we store the field which produces the pulse with the highest yield and consider this field as the result of the optimization.
% 
\end{itemize}



==> comp_details.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\section{Computational details and model system}
\label{sec:compdetails}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
We choose a one-dimensional asymmetric double well to test our algorithms. The double well is similar to reference \cite{GH98} but has an additional  cubic term:
%
\begin{eqnarray}
%
V(x) = \frac{w_0^4}{64 B} x^4 -  \frac{\omega_0^2}{4} x^2 + \beta x^3 ,
%
\end{eqnarray} 
%
with $\omega_0$ corresponding to the classical frequency at the bottom of the well and the parameter $B$ adjusting the barrier height. The number of pairs of states below the barrier is approximately $B/\omega_0$. Here, we choose $B=\omega_0=1.0$ and $\beta=1/256$ which leads to two states below the barrier, as shown in \fref{fig:potential_states}.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering
\includegraphics*[width=.43\textwidth]{fig1.eps}       

\caption{The plot shows the model potential with the ground state (\full), the first excited state (\dashed), the second excited state (\dotted) and the third excited state (\chain). Each state is shifted according to its eigenvalue.} 
\label{fig:potential_states}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%some numbers
In order to analyze the laser pulses from the optimization runs we calculate the excitation energies (see \tref{tab:xenergies}) and dipole moments (see \tref{tab:dipole_moments}) of the system by propagating in imaginary time.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\begin{indented}
\item[]
\caption{\label{tab:xenergies}Excitation energies in atomic units~[a.u.] for the 1D asymmetric double well, calculated by imaginary time propagation.}
\lineup
\begin{tabular}{@{}lllll}
\br  
 & $|0\rangle$        & $|1\rangle$         & $|2\rangle$        & $|3\rangle$      \\% &  4      & 5  \\ 
\mr
 $|0\rangle$   & 0.       &           &          &         \\% &         &      \\  
 $|1\rangle$   & 0.1568  &  0.       &          &         \\% &         &      \\
 $|2\rangle$   & 0.7022  &  0.5454  & 0.       &         \\% &         &     \\ 
 $|3\rangle$   & 1.0147  &  0.8580  & 0.3125  & 0.      \\% &        \\ &    \\
 $|4\rangle$   & 1.5294  &  1.3726  & 0.8273  & 0.5147 \\% & 0.    \\%  &     \\
\br
\end{tabular}
\end{indented}
\end{table}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\begin{indented}
\item[]
\caption{\label{tab:dipole_moments}Dipole matrix elements for the 1D asymmetric double well, calculated by imaginary time propagation.}
%\lineup
\begin{tabular}{@{}ld{4}d{4}d{4}d{4}d{4}}
\br
    &  |0\rangle       & |1\rangle        & |2\rangle        &  |3\rangle       &  |4\rangle  \\
\mr
  $|0\rangle$   & -2.5676  &         &         &         &        \\
  $|1\rangle$   &  0.3921  &  2.3242 &         &         &        \\
  $|2\rangle$   &  0.6382  & -0.7037 & -0.5988 &         &        \\
  $|3\rangle$   & -0.3865  & -0.4630 &  1.7051 &  0.1958 &        \\
  $|4\rangle$   & -0.1414  &  0.2118 &  0.1593 & -1.7862 & -0.0939 \\
\br
\end{tabular}
\end{indented}
\end{table}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TDSE

The time-dependent Schr\"odinger equation for the 1D double well is solved on an equidistant grid, where the infinitesimal time-evolution operator is approximated by the 2nd-order split-operator (SPO) technique \cite{FMF76}:
%
\begin{eqnarray} 
%
\nonumber
%
\widehat{U}_{t}^{t+\Delta t}&=&\mathcal{T}\exp\left(-i \int_{t}^{t+\Delta t} \!\! dt' \,\, \widehat{H}(t')\right)\\
%
\nonumber
%
\label{eq:spo2nd}
    & \approx  & \exp(-\frac{i}{2}\, \hat {T}\,\Delta t) \exp(-i\, \hat {V}(t)\,\Delta t)\times 
    \exp(-\frac{i}{2}\, \hat {T}\,\Delta t) + O(\Delta t^3).
%
\end{eqnarray}
%
%
Following the scheme described in \sref{algorithm}, one needs three propagations per iteration (if we want to avoid storing the wave function). Within the 2nd order split-operator scheme each time step requires 4 Fast Fourier Transforms (FFT) \cite{FFTW98} for the backward propagations, because we have to know the wave-function and the Lagrange multiplier in real space at every time-step to be able to evaluate the field from equation \eref{eq:field}. For the forward propagation we only need 2 FFTs. This sums up to $10$ FFTs per time step and iteration. \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\begin{indented}
\item[]
\caption{\label{tab:parameter}In ordinary runs the listed numerical parameters (given in atomic units) were employed. For the scans in \sref{sec:scan} we have used a coarser grid in space and time, as indicated in the second column.}
%\lineup
\begin{tabular}{@{}ld{4}d{4}l}
\br
parameter     & \mbox{single run} & \mbox{scan} & \\
\mr
$T$           & 400.0 & 400.0  & pulse length  \\   
$x_{\mathrm{max}}$  & 30.0 & 20.0 & grid size \\
$dx$          & 0.1172  & 0.1563 & grid spacing \\
$dt$          & 0.001  & 0.005 & time step \\
$\epsilon^{(0)}$         & -0.2  & -0.2 & initial guess \\
\br
\end{tabular}
\end{indented}
\end{table}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The parameters used in the runs are summarized in \tref{tab:parameter}. The initial guess for the laser field was $\epsilon^{(0)}(t)=-0.2$ in all calculations. This choice is arbitrary but has the advantage of producing a significant occupation in the target state at the end of the pulse, necessary to get the iteration working. Although the simple choice $\epsilon^{(0)}(t)=0.0$ will work as well in most cases, it represents a minimum of the functional since initial and target state are orthonormal. Therefore the algorithm could get stuck in principle.
The obtained solutions, which are presented in the following chapter, are all far away from the initial guess. This suggests that the solutions do not depend on the initial guess for the laser field. 
%


==> results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results}
\label{sec:results}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In this section we apply the algorithms described above to our 1D model for electron transfer. We start in the ground state $| 0 \rangle$ ($t=0$) where the electron is localized in the left well and demand that at the end of the laser pulse ($t=T$) it will be transfered to 1st excited state $|1 \rangle$, which is mainly located in the right well (see \fref{fig:potential_states}). The target operator in this case is a projection operator onto the first excited state: $\widehat{O} = | 1 \rangle \langle 1 |$. Therefore, the success is measured by $| \langle \Psi(T) | 1 \rangle |^2$ which we simply refer to as the ``yield''.
The pulse length is chosen to be $T=400$ ($\approx 9.7$~fs).

%%
%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Fluence constraints} \label{sec:fluence}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Fixed fluence.}\label{sec:fluence_2lev}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In the following we first apply our algorithm to find an optimal field with the fluence $E_0=0.080$. This is the value obtained by an estimate using the two-level system (see \ref{app_2lev}). After $894$ iterations we obtain a yield of $99.91\%$ which is higher than the yield found by the two-level estimate. The optimal laser field and its spectrum (Fourier transform) are shown in figures \ref{fig:field_E1} and \ref{fig:field_E2}. The spectrum is dominated by three narrow peaks which correspond to the excitation energies $\omega_{01}=0.156$, $\omega_{12}=0.545$ and $\omega_{02}=0.702$. This suggests that the optimized transition process is a mixture of the direct process, i.e. the excitation from $|0\rangle \to |1\rangle$ and an indirect process which uses the second excited state as intermediate state: $|0\rangle \to |2\rangle \to |1\rangle $. Other indirect processes, like $|0\rangle \to |3\rangle \to |1\rangle $, play only a minor role in this case. This interpretation is supported by looking at the evolution of the occupation numbers in time (\fref{fig:field_E3}). First, the laser pulse populates the second excited state (\dotted) and then after half of the pulse duration depopulates it again.  
Looking once more at the spectrum (in \fref{fig:field_E2}) we observe a group of peaks around $\omega_{01}$ 
%
($\omega\in [0,0.1]$ and $\omega \in [0.2,0.3]$) 
%
which do not correspond to any excitation energy of the field-free Hamiltonian. However, these frequencies play an important role in the transition process. If we filter out these frequency components, rescale the fluence to $E_0=0.080$, and then propagate this modified laser pulse, we find, at the end of the pulse, the following occupations: ground-state $16\%$, first excited state $38\%$, second excited state: $44\%$, and in all higher levels $6\%$. In particular, the direct transition and the back transfer from the intermediate level $|2 \rangle $ to the target state in the indirect process are less efficient without these extra frequencies. Further analysis of this kind shows that the low-frequency components and especially the zero frequency component (bias) are crucial since they introduce a (slight) shift of the resonance frequencies, visible as a broadening of the $\omega_{01}$ peak in \fref{fig:field_E2}. If, on the other hand, these components are missing the remaining frequencies become slightly off-resonant, resulting in the low efficiency of $44\%$.   

If we filter out everything except the extra peaks we find a target state occupation of $1\%$. Understanding these extra peaks as a third type of transfer process (see \sref{sec:lowfrequency}) suggests that, in this case, a mixing of transition processes seems to be superior in terms of the maximum target yield than a pulse consisting of a single process only, e.g. the direct process. %The complication that the third type process requires the frequency components (for the direct and indirect transition) to be shifted, is easily resolved by the algorithm.

The final yield $99.91\%$ is only $0.61\%$ better than the yield coming from the simple monochromatic pulse estimate of the two-level system. This gain has a high price, the optimized pulse is hardly realizable in any experiment. Although the gain improves with shorter pulse lengths (see \ref{app_2lev}), this example demonstrates the typical dilemma between theory and experiment: Calculated pulses often have a far too complicated spectrum to be produced in practice. In \sref{sec:spectral} and \ref{sec:combination} we demonstrate how this dilemma can be resolved.
%The frequencies can be explained by calculating the differences between the two lowest eigenvalues of the Hamiltonian including the laser field at each point in time. These values oscillate between $0.02$ and $0.30$ around $\omega_{01}$ which explains the appearance of the ``off-resonant'' peaks.

To conclude the analysis we look at the convergence behavior of the applied scheme (see \fref{fig:field_E4}). We find a fast convergence within the first 20 iterations. After these 20 iterations the improvement of the yield slows down, like it is also found in the rapid monotonic schemes presented in references \cite{ZBR98,MT2003}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering 
\subfigure[]{
  \label{fig:field_E1}
      \includegraphics*[width=.33\textwidth]{fig2a.eps}
      %\hspace{.3in}
    }
\subfigure[]{
  \label{fig:field_E2}
  \includegraphics*[width=.33\textwidth]{fig2b.eps}
  %\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_E3}
  \includegraphics*[width=.33\textwidth]{fig2c.eps}
  %\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_E4}
  \includegraphics*[width=.33\textwidth]{fig2d.eps} 
%hspace{.3in}
}
\caption{We apply the algorithm for $E_0=0.080$. The optimized field is shown in (a), with its spectrum in (b). In (c) we plot the time evolution of the occupation numbers $|\langle \Psi(t) | n \rangle |^2$ ($n=0$ (\full), $n=1$ (\dashed), $n=2$ (\dotted) and $n=3$ (\chain)). The convergence behavior is shown in (d). Also shown in (d) are the values of the Lagrange multiplier $\alpha$ (\dashed) during the iteration which we scaled by a factor of $0.1$. The \opencircle indicates the iteration with the highest yield.}
\label{fig:field_E}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Energy versus yield}
\label{sec:scan}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

We apply our method to scan through a range of values for $E_0$ from $0.010 \ldots 1.000$. 
The scan, displayed in \fref{fig:scan_En}, shows that there seems to be a critical value $\tilde{E}_0$ which is necessary to get very high occupations ($|\langle \Psi(T)|1 \rangle |^2 > 0.99$ of the target state. For values $E_0>\tilde{E}_0$ the algorithm always finds a laser field that produces yields above $99\%$.

For long pulse durations (as it is the case here) we can give a rough estimate of this critical value  $\tilde{E}_0$  with the help of the two-level system:
\begin{eqnarray}
\tilde{E}_0 &\approx & A^2 \frac{T}{2} = \frac{\pi^2}{2 \mu_{01}^2 T }\\
%
\end{eqnarray}
%
with $A =  \pi / \left(\mu_{01} T\right)$ (see \ref{app_2lev}).
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering
\includegraphics*[width=.43\textwidth]{fig3.eps}       
\caption{The graph shows the yield for different values of $E_0$ ranging from $0.010$ to $1.000$. Each point corresponds to a single optimization. For these runs we have used a smaller grid ($x_{max}=-x_{min}=20.0$, $dx=0.15625$) and a larger time-step ($dt=0.005$). The vertical line (\dashed) corresponds to $E_0=0.080$. Beyond this line only yields higher than $0.99$ are found.} 
\label{fig:scan_En}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

If we take a closer look at some of the optimized fields (see \fref{fig:fields_Escan1}) for the values  $E_0=0.010,0.050,0.100,0.200$, we see that the spectra (see \fref{fig:fields_Escan2}) of these pulses get more complicated as the assigned fluence increases. In the lower two panels ($E_0=0.010,0.050$) we find peaks at the exact resonance frequencies. The optimized fields result in occupations of $35.24\%$ and $97.63\%$. While the pulses shown in the two upper panels ($E_0=0.100,0.200$) produce yields of $99.81\%$ and $99.95\%$. The peaks corresponding to the direct $|0\rangle \to |1 \rangle$  and indirect process $|0\rangle \to |2 \rangle \to |1\rangle $ are ``Stark'' shifted. For the stronger pulses, we also find an increasing low-frequency part. The spectrum in the top panel ($E_0=0.200$) is difficult to analyze. However, one can see that more and more processes are taking part in the transition, i.e. peaks occur near the other resonance frequencies.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering 
\subfigure[]{
  \label{fig:fields_Escan1}
      \includegraphics*[width=.4\textwidth]{fig4a.eps}
      \hspace{.3in}
    }
\subfigure[]{
  \label{fig:fields_Escan2}
  \includegraphics*[width=.4\textwidth]{fig4b.eps}
\hspace{.3in}
}
\caption{In (a), we plot the optimized laser fields for different values of $E_0={ 0.010, 0.050, 0.100, 0.200 }$. Graph (b) shows the corresponding spectra. The resonance frequencies for the transitions $|0 \rangle \to |1 \rangle$, $|1 \rangle \to |2 \rangle$ and  $|0 \rangle \to |2 \rangle$  are indicated by vertical lines. In the two upper plots of graph (b) the peaks are Stark-shifted. Note, that these spectra also contain a large low frequency part.}
\label{fig:fields_Escan}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Spectral constraints} \label{sec:spectral}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
In the following we present the results of the algorithm with spectral constraints and penalty factor for two examples of the filter function. These examples are motivated by the findings of the previous chapter, namely that the transfer of the particle occurred via a mixture of a direct transition and indirect transitions. We want to find a laser pulse that produces a high yield and only contains spectral components centered around the resonance frequency $\omega_{01}$. We know that such a pulse exists, since it appeared in the second iteration when looking for a pulse with $E_0=0.080$ (see \sref{sec:fluence_2lev}). 
In the second example we optimize a laser that is not allowed to contain the excitation frequency $\omega_{01}$ of the direct process.

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Direct transition} \label{sec:direct}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Using spectral constraints in the optimization scheme allows us to explicitly select the direct transition, i.e. we search for a pulse whose main frequency component is the excitation energy $\omega_{01}$. This is done by applying a Gaussian shaped frequency filter $f(\omega)$, according to equation \eref{eq:filter1}, centered around $\omega_0 = \omega_{01}$ and with $\gamma=500$.  

After $50$ iterations the algorithm finds a laser pulse which results in a yield of $99.97\%$ . We set the penalty factor $\alpha=0.05$ and obtain a value of $E_0 = 0.090$ which is slightly higher than the estimate from the two-level model but also more effective.
The slight envelope on the field, shown in \fref{fig:field_F1}, stems from the finite width of the Gaussian (see \fref{fig:field_F2}). Frequency components near $\omega_{01}$ are still allowed in the pulse and result in a beat pattern. The time dependent occupation numbers confirm that the higher states are not occupied during the transition (see \fref{fig:field_F3}). The convergence, shown in \fref{fig:field_F3} is rather smooth.
Note, that if we desire a sinusoidal field with a constant envelope we have to reduce the width of the Gaussian to allow only one single component in the spectrum (a Kronecker delta). Using such a filter we obtain a yield of $99.79\%$ and $E_0=0.085$. The field oscillates with the amplitude $A=0.0207$ which is slightly higher than the amplitude derived from the two-level system (see \ref{app_2lev}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering 
\subfigure[]{
  \label{fig:field_F1}
      \includegraphics*[width=.33\textwidth]{fig5a.eps}
   %   \hspace{.3in}
    }
\subfigure[]{
  \label{fig:field_F2}
  \includegraphics*[width=.33\textwidth]{fig5b.eps}
%\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_F3}
  \includegraphics*[width=.33\textwidth]{fig5c.eps}
%\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_F4}
  \includegraphics*[width=.33\textwidth]{fig5d.eps}
%\hspace{.3in}
}

\caption{We apply the optimization algorithm but allowing only a Gaussian frequency distribution around $\omega_{01}=0.1568$. The resulting field is displayed in graph (a). The filter function $f(\omega)$ (\dashed) which is scaled by $0.01$ is shown together with the spectrum in (b). The time dependent occupation numbers (c) confirm that only the ground state (\full) and the first excited state (\dashed) take part in the process. The second excited state population (\dotted) is hardly visible. The convergence is shown in graph (d). The \opencircle indicates the iteration with the highest yield.}
\label{fig:field_F}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Forbidden direct transition} \label{sec:forbid_direct}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
By choosing the complement of the filter function from the previous example, i.e., by allowing every frequency component except $\omega_{01}$, we can optimize a field which also produces a very high yield. The filter function is given by equation \eref{eq:filter2} with $\omega_{0} = \omega_{01}$ and $\gamma=500$.

The optimization procedure (with a penalty factor $\alpha=2.5$) results in a target state occupation of $99.60\%$ after $269$ iterations. The optimized laser field is presented in \fref{fig:field_FC1}, it integrates to a fluence of $E_0=0.130$. Its spectrum, shown in \fref{fig:field_FC2}, consists of two major components: $\omega_a=0.581$ and $\omega_b=0.676$ which correspond to the Stark-shifted excitation energies $\omega_{12}$ and $\omega_{02}$, i.e. the optimization takes care of the frequency shifts introduced by the large bias (zero-frequency component) of the field. That the transition occurs via the indirect process is confirmed by looking at the time-dependent occupation numbers, shown in \fref{fig:field_FC3}. First, the field starts populating the second excited state and then transfers the population to the target state. Other indirect processes, e.g. $|0\rangle \to |3\rangle \to  |1\rangle$ or $|0\rangle \to |2\rangle \to  |3\rangle \to |1\rangle $, 
play only a minor role: The occupation of the third excited state stays below $2.5\%$ and the frequency components correponding to these processes are very small.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering 
\subfigure[]{
  \label{fig:field_FC1}
      \includegraphics*[width=.33\textwidth]{fig6a.eps}
%      \hspace{.3in}
    }
\subfigure[]{
  \label{fig:field_FC2}
  \includegraphics*[width=.33\textwidth]{fig6b.eps}
%\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_FC3}
  \includegraphics*[width=.33\textwidth]{fig6c.eps}
%\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_FC4}
  \includegraphics*[width=.33\textwidth]{fig6d.eps}
%\hspace{.3in}
}

\caption{We prohibit the direct transition from $|0 \rangle \to |1 \rangle $ by using the complement of the previous filter function $\tilde{f}(\omega) = 1 -f(\omega)$. The optimized field is shown in graph (a). The filter function $\tilde{f}(\omega)$ (\dashed), scaled by $0.01$, is plotted together with the spectrum in (b). The time-dependent occupation numbers (c) confirm that now the second excited state (\dotted) plays a major role in the transition (ground state (\full), first-excited state (\dashed) and third excited state (\chain)).  The convergence is shown in graph (d). The \opencircle indicates the iteration with largest occupation of the target-state.}
\label{fig:field_FC}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Combination of Spectral and fluence constraints}
\label{sec:combination}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The next examples demonstrate that even more restrictions are possible and we can still obtain very good yields. We combine the spectral restriction with the fluence constraint and continue the above examples by  selecting among the indirect processes. Only two frequencies are allowed in the laser pulse and in addition we fix the fluence.
In the last example we show that it is not even necessary to have resonance frequencies inside the laser pulse to reach very high occupations of the target state. 

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Selective transfer via intermediate state $| 2 \rangle$} 
\label{sec:indirect021}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In the former examples we found that the indirect process $|0\rangle \to |2\rangle \to |1\rangle$ plays a major role in the excitation process. Since it appeared always together with other processes, e.g. in \sref{sec:fluence_2lev} together with the direct process or in \sref{sec:forbid_direct} together with other indirect processes, we try to find a laser field with only the two excitation energies $\omega_{02}$ and $\omega_{12}$ ($\gamma=500$) and in addition require $E_0=0.160$. For these high requirements we have to pay a price which is the irregular behaviour of the yield during the iteration, shown in \fref{fig:field_FC021_4}. After $540$ iterations we find a yield of $99.90\%$. 
The restriction of the laser frequencies results exactly in the desired transition process, which is confirmed by the time-dependent occupation numbers, shown in \fref{fig:field_FC021_3}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering 
\subfigure[]{
  \label{fig:field_FC021_1}
      \includegraphics*[width=.33\textwidth]{fig7a.eps}
 %     \hspace{.3in}
    }
\subfigure[]{
  \label{fig:field_FC021_2}
  \includegraphics*[width=.33\textwidth]{fig7b.eps}
%\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_FC021_3}
  \includegraphics*[width=.33\textwidth]{fig7c.eps}
%\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_FC021_4}
  \includegraphics*[width=.33\textwidth]{fig7d.eps}
%\hspace{.3in}
}

\caption{Here we use a double gaussian window ($\gamma=500$), allowing only frequencies around $\omega_{02}$ and $\omega_{21}$ and in addition demand $E_0=0.160$. The optimized field is shown in graph (a). The filter function (\dashed) $f(\omega)$, scaled by $0.01$, is plotted together with the spectrum in (b). The time-dependent occupation numbers  (ground state (\full), first-excited state (\dashed) and third excited state (\chain)) in (c) confirm that the transition occurs via the second excited state (\dotted). Due to the stronger constraints the convergence behaviour becomes oscillatory, shown in graph (d). }
\label{fig:field_FC021}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Selective transfer via intermediate state $| 3 \rangle$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The process $|0\rangle \to |3\rangle \to |1\rangle$ using the third excited state as intermediate state played only a minor role in the examples considered so far. Here, we try to optimize the laser pulse so that the transition is only performed via this process. In addition we require $E_0=0.320$. 
Again, we use a double Gaussian filter, one Gaussian centered at $\omega_{13}$, the other one at $\omega_{03}$ and choose the width parameter $\gamma=500$.
 
The results are shown in \fref{fig:field_FC031}. Like in the previous example, the high requirements on the laser field result in a rather erratic convergence (see \fref{fig:field_FC031_4}). The field, shown in \fref{fig:field_FC031_1}, produces a target state occupation of $99.89\%$ after $162$ iterations. The time-dependent occupation numbers (see \fref{fig:field_FC031_3}) show that the transition happens exactly in the desired way.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering 
\subfigure[]{
  \label{fig:field_FC031_1}
      \includegraphics*[width=.33\textwidth]{fig8a.eps}
%      \hspace{.3in}
    }
\subfigure[]{
  \label{fig:field_FC031_2}
  \includegraphics*[width=.33\textwidth]{fig8b.eps}
%\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_FC031_3}
  \includegraphics*[width=.33\textwidth]{fig8c.eps}
%\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_FC031_4}
  \includegraphics*[width=.33\textwidth]{fig8d.eps}
%\hspace{.3in}
}

\caption{We apply the optimization algorithm with a double gaussian window, allowing only frequencies around $\omega_{03}$ and $\omega_{31}$ and in addition set $E_0=0.320$. The optimized field is shown in graph (a). The filter function $f(\omega)$ (\dashed), scaled by $0.01$, is plotted together with the spectrum (b). The time-dependent occupation numbers (ground state (\full), first-excited state (\dashed) and second excited state (\dotted)), shown in (c), confirm that the transition process is performed mainly via the third excited state (\chain). Due to the strong restrictions the convergence behaviour happens to be more oscillatory, shown in graph (d). }
\label{fig:field_FC031}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Low frequency pulse}
\label{sec:lowfrequency}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Using a band filter, i.e. $f(\omega) = \theta(\omega - \omega_a)* \theta(\omega_b - \omega) +  \theta(-\omega_a - \omega)* \theta(\omega + \omega_b)$, with $\omega_a = 0.000$ and $\omega_b=0.120$ we can find a laser pulse resulting in high yields without allowing any resonance frequency in the laser spectrum. The allowed frequencies ($\omega \in [0.000,0.120]$) are smaller than the lowest excitation frequency $\omega_{01}$. The additional constraint on the fluence in the optimization is $E_0=0.400$. 
The convergence of this optimization is shown in \fref{fig:field_S4}. After $981$ iterations, we obtain a target state occupation of $99.93\%$. The spectrum of the optimized pulse, shown in \fref{fig:field_S2}, exhibits contributions of all allowed frequency components. In particular, the zero-frequency component is dominant, being almost three times larger than the other frequency contributions. In the time-domain the zero-frequency component corresponds to a bias of $\epsilon_{\mathrm{av}}=-0.028$ which is close to the value for which the potential becomes almost symmetric: $\bar{\epsilon}=-0.031$. The optimized pulse together with $\bar{\epsilon}$ are shown in the middle panel of \fref{fig:fieldS1}. 

The transfer process can be interpreted with the help of the following simplified picture: Assume the field would be almost static with $\epsilon(t) \approx \bar{\epsilon}$. Then, the initial state becomes a superposition of the dressed states
%
\begin{eqnarray}
\nonumber
\Psi(x,t=0) = \frac{1} {\sqrt{2}} \left( \varphi_0^{\mathrm{\bar{\epsilon}}} - \varphi_1^{\mathrm{\bar{\epsilon}}}\right) e^{i \theta_1}. 
\end{eqnarray}
%
Small perturbations of the laser field around $\bar{\epsilon}$ rearrange the phases of the superposition so that at the end of the pulse
%
\begin{eqnarray}
\nonumber
\Psi(x,T) =  \frac{1} {\sqrt{2}} \left(\varphi_0^{\mathrm{\bar{\epsilon}}} + \varphi_1^{\mathrm{\bar{\epsilon}}}\right)e^{i \theta_2}. 
\end{eqnarray}
%
This superposition is located in the right well which completes the transfer. Note, that the phases $\theta_1$, $\theta_2$ are irrelevant in this case.

The pulse we have obtained from the optimization is more difficult to explain since the oscillations around $\bar{\epsilon}$ are not small. To be able to analyse the transfer process in similar terms as discussed above, we have calculated the projections of the wave function $\Psi(x,t)$ onto the eigenfunctions of the Hamiltonian $\hat{H}^{\bar{\epsilon}}$ including the field $\bar{\epsilon}$. These ``dressed'' occupation numbers are shown in the upper panel of \fref{fig:fieldS1}.
In the simplified interpretation we have implicitly assumed a complete localization in the left (right) well for the initial (target) state. Since this is not true for the potential chosen here, the dressed occupation numbers deviate slightly from $0.5$, namely we have $|\langle \Psi(x,0) | \varphi_0^{\bar{\epsilon}} \rangle|^2 = 0.57$  and $|\langle \Psi(x,0) | \varphi_1^{\bar{\epsilon}} \rangle|^2 = 0.43$. At the end of the pulse we obtain the inverted occupation numbers, i.e. $|\langle \Psi(x,T) | \varphi_0^{\bar{\epsilon}} \rangle|^2 = 0.45$ and $|\langle \Psi(x,T) | \varphi_1^{\bar{\epsilon}} \rangle|^2 = 0.55$ which indicates the completed transfer (necessary condition). The laser pulse has also adjusted the phases of the expansion coefficients in the right way (sufficient condition): The relative phase difference of $\phi_0^{\mathrm{\bar{\epsilon}}}$ and $\phi_1^{\mathrm{\bar{\epsilon}}}$ between $t=0$ and $t=T$ was found to be $0.8*\pi$. This deviates from the simple picture where we would have expected a phase difference of $\pi$.

The transfer process described above has similarities with the one discovered in reference \cite{DKMS98} where the authors have used an asymmetric double well to model a hydrogen transfer reaction. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering
\includegraphics*[width=.45\textwidth]{fig9.eps}
\caption{In the lower panel we show the time-dependent occupation numbers of the ground-state (\full), the first excited state (\dashed) and the second excited state (\dotted).  The optimized laser field together with $\bar{\epsilon}=-0.031$ is shown in the middle panel. In the top panel we plot the absolute values (squared) of the projections onto the two lowest eigenfunctions of the Hamiltonian including the field $\bar{\epsilon}$.}
\label{fig:fieldS1}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
\centering 
\subfigure[]{
  \label{fig:field_S2}
  \includegraphics*[width=.33\textwidth]{fig10a.eps}
%\hspace{.3in}
}
\subfigure[]{
  \label{fig:field_S4}
  \includegraphics*[width=.33\textwidth]{fig10b.eps}
%\hspace{.3in}
}
\caption{ Graph (a) shows the spectrum of the laser field (\full) and the rectangular filter (\dashed) scaled by $0.01$. The convergence is shown in (b). The \opencircle indicates the iteration with the highest yield.}
\label{fig:field_S}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
